Estimating the Number of Fatal Victims of the Peruvian Internal Armed Conflict, 1980-2000: an application of modern multi-list Capture-Recapture techniques

We estimate the number of fatal victims of the Peruvian internal armed conflict between 1980-2000 using stratified seven-list Capture-Recapture methods based on Dirichlet process mixtures, which we extend to accommodate incomplete stratification information. We use matched data from six sources, originally analyzed by the Peruvian Truth and Reconciliation Commission in 2003, together with a new large dataset, originally published in 2006 by the Peruvian government. We deal with missing stratification labels by developing a general framework and estimation methods based on MCMC sampling for jointly fitting generic Bayesian Capture-Recapture models and the missing labels. Through a detailed exploration driven by domain-knowledge, modeling and refining, with special precautions to avoid cherry-picking of results, we arrive to a conservative posterior estimate of 58,234 (CI95% = [56,741, 61,289]), and a more liberal estimate of 65,958 (CI95% = [61,462, 75,387]) fatal victims. We also determine that the Shining Path guerrillas killed more people than the Peruvian armed forces. We additionally explore and discuss estimates based on log-linear modeling and multiple-imputation. We finish by discussing several lessons learned about the use of Capture-Recapture methods for estimating casualties in conflicts.

==> MI_LCMCR_26strata.tex <==
% latex table generated in R 3.5.3 by xtable 1.8-3 package
% Mon May 13 10:26:46 2019
\begin{table}[tbp]
\centering
\begin{tabular}{lrrrr}
 Perpetrator & $n$ & $\hat n_\text{IMP}$ & $\hat N$ & $CI_{95\%}$ \\ 
  \hline
Peruvian State (EST) & 12,901 & 1,087 & 27,254 & [22,878, 33,677] \\ 
  Shinning Path (SLU) & 17,687 & 1,949 & 35,250 & [31,847, 39,594] \\ 
  Other (OTR) & 1,158 & 180 & 2,202 & [1,867, 2,689] \\ 
   \hline
Total & 31,746 & 3,216 & 65,013 & [58,709, 72,938] \\ 
  \end{tabular}
\caption{Multiple imputation LCMCR estimates of population size aggregated by perpetrator. Estimates were computed stratifying by perpetrator and geographic region (26-region scheme). Estimates are combined posterior medians. Column $\hat n_\text{OTR}$ contains estimates of the number of records from NOD that correspond to each perpetrator; its total coincides with the total of records originally labeled ``NOD".} 
\label{tab:MI:LCMCR:26strata}
\end{table}


==> capture_patterns.tex <==
% latex table generated in R 3.5.3 by xtable 1.8-3 package
% Mon May 13 10:26:18 2019
\begin{tabular}{rrrrrrrr}
 CVR & DP & CEDAP & CNDDHH & COMISEDH & CICR & MIMDES & $n$ \\ 
  \hline
0 & 0 & 0 & 0 & 0 & 0 & 1 & 13018 \\ 
  1 & 0 & 0 & 0 & 0 & 0 & 0 & 9094 \\ 
  1 & 0 & 0 & 0 & 0 & 0 & 1 & 5752 \\ 
  0 & 0 & 0 & 0 & 1 & 0 & 0 & 726 \\ 
  0 & 1 & 0 & 0 & 1 & 0 & 0 & 708 \\ 
  0 & 1 & 0 & 0 & 0 & 0 & 0 & 621 \\ 
  0 & 0 & 1 & 0 & 0 & 0 & 0 & 549 \\ 
  1 & 1 & 0 & 0 & 0 & 0 & 0 & 370 \\ 
  0 & 0 & 0 & 1 & 0 & 0 & 0 & 320 \\ 
  1 & 1 & 0 & 1 & 1 & 0 & 0 & 307 \\ 
  \end{tabular}


==> fit_loglin_MI17.tex <==
% latex table generated in R 3.5.3 by xtable 1.8-3 package
% Mon May 13 10:27:07 2019
\begin{table}[tbp]
\centering
\begin{tabular}{lrrrr}
 Loglin Fit? & Strata & $\hat N_\text{loglin}$ & $\hat N_\text{LCMCR}$ & $\hat N_\text{loglin}$ - $\hat N_\text{LCMCR}$ \\ 
  \hline
No & 54 & 43,692 & 37,916 & 5,776 \\ 
  Yes & 24 & 25,384 & 24,840 & 544 \\ 
   \hline
Total & 78 & 69,076 & 62,756 & 6,320 \\ 
  \end{tabular}
\caption{Log-linear and LCMCR estimates for imputation \#17 by fit of selected log-linear 
         models used to estimate each stratum. Models with deviance-based p-value $\geq 0.05$ 
         are considered to fit the data. Estimates come from the aggregation of 78 strata. Most of the difference 
         between log-linear and LCMCR estimates (8,544) is concentrated in strata where it 
         was  not possible to find a good fitting log-linear model.} 
\label{tab:fit:loglin:MI:17}
\end{table}


==> unstratified_perp.tex <==
% latex table generated in R 3.5.3 by xtable 1.8-3 package
% Mon May 13 10:26:25 2019
\begin{tabular}{lrrr}
 Perpetrator & $n$ & $\hat{N}$ & $CI_{95\%}$ \\ 
  \hline
Peruvian State (EST) & 12,052 & 33,840 & (*)[25,894, 46,552] \\ 
  Shinning Path (SLU) & 17,519 & 28,940 & [28,239, 30,120] \\ 
  Other (OTR) & 1,120 & 2,307 & [2,069, 2,601] \\ 
  Undetermined (NOD) & 3,212 & 11,206 & (*)[7,791, 43,241] \\ 
   \hline
TOTAL & 33,903 & 80,562 & [67,470, 111,808] \\ 
  \end{tabular}

